Seamless Multimodal Biometrics for Continuous Personalised Wellbeing Monitoring

Artificially intelligent perception is increasingly present in the lives of every one of us. Vehicles are no exception, (...) In the near future, pattern recognition will have an even stronger role in vehicles, as self-driving cars will require automated ways to understand what is happening around (and within) them and act accordingly. (...) This doctoral work focused on advancing in-vehicle sensing through the research of novel computer vision and pattern recognition methodologies for both biometrics and wellbeing monitoring. The main focus has been on electrocardiogram (ECG) biometrics, a trait well-known for its potential for seamless driver monitoring. Major efforts were devoted to achieving improved performance in identification and identity verification in off-the-person scenarios, well-known for increased noise and variability. Here, end-to-end deep learning ECG biometric solutions were proposed and important topics were addressed such as cross-database and long-term performance, waveform relevance through explainability, and interlead conversion. Face biometrics, a natural complement to the ECG in seamless unconstrained scenarios, was also studied in this work. The open challenges of masked face recognition and interpretability in biometrics were tackled in an effort to evolve towards algorithms that are more transparent, trustworthy, and robust to significant occlusions. Within the topic of wellbeing monitoring, improved solutions to multimodal emotion recognition in groups of people and activity/violence recognition in in-vehicle scenarios were proposed. At last, we also proposed a novel way to learn template security within end-to-end models, dismissing additional separate encryption processes, and a self-supervised learning approach tailored to sequential data, in order to ensure data security and optimal performance. (...)

==> Makefile <==
#
# Makefile for feupteses/feupthesis
#
# Version:   Sat May 17 22:36:50 2008
# Written by JCL
#

## programs
LATEX=latex
PDFLATEX=pdflatex
BIBTEX=bibtex
DVIDVI=dvidvi -m '2:0(3mm,-14mm),1(193mm,-14mm)'
DVIPS=dvips -Ppdf
DVI2PS=dvips -t landscape -x 707
PS2PDF=ps2pdf -dEmbedAllFonts#true
MKIDX=makeindex

## Basename for result in PT
TARGET:=tese-pt
## Basename for result in EN
#TARGET:=thesis-en

# Basename for result in PT: PDI
#TARGET:=pdi-pt

# Basename for result in PT: PDI
# TARGET:=pdi-en

## .tex files
TEXFILES=$(wildcard *.tex **/*.tex)

## BibTeX files
BIB=$(wildcard *.bib)

## paper
PAPERSIZE=a4

#we prefer pdflatex for bibtex
LATEXBIB=$(PDFLATEX)

main:	$(TARGET).pdf

index:
	$(MKIDX) $(TARGET)

biblio:
	$(BIBTEX) $(TARGET)

.tex.pdf:
	rm -f $(TARGET).pdf
	$(PDFLATEX) $< $@ || { rm -f $*.aux $*.idx && false ; }
	if grep 'There were undefined references' $*.log ; then \
	  $(BIBTEX) $(TARGET); $(PDFLATEX) $< $@; fi
	while grep 'Rerun to get cross-references right.' $*.log ; do \
	  $(PDFLATEX) $< $@ || { rm -f $*.aux $*.idx && false ; } ; done

.tex.dvi:
	rm -f $*.ps $*.pdf
	$(LATEX) $< || { rm -f $*.dvi $*.aux $*.idx && false ; }
	if grep 'There were undefined references' $*.log ; then \
	  $(BIBTEX) $(TARGET); $(LATEX) $< $@; fi
	while grep 'Rerun to get cross-references right.' $*.log ; do \
	  $(LATEX) $< || { rm -f $*.dvi $*.aux $*.idx && false ; } ; done

.dvi.ps:
	$(DVIPS) -t $(PAPERSIZE) $< -o $@

.dvi.dvi2:
	$(DVIDVI) $< $@

.dvi2.ps2:
	$(DVI2PS) $< -o $@

.ps.pdf:
	$(PS2PDF) $< $@

.bib.bbl:
# in case we don't already have a .aux file listing citations
	$(LATEXBIB) $(TARGET).tex
# get the citations out of the bibliography
	$(BIBTEX) $(TARGET)
# do it again in case there are out-of-order cross-references
	$(LATEXBIB) $(TARGET).tex
	$(BIBTEX) $(TARGET)

$(TARGET).pdf:	  $(TEXFILES)
$(TARGET).dvi:	  $(TEXFILES)
$(TARGET).ps:	  $(TARGET).dvi
$(TARGET).ps2:	  $(TARGET).dvi2
$(TARGET).dvi2:	  $(TARGET).dvi

## Extensions
EXTS=aux toc idx ind ilg log out lof lot lol bbl blg

##clean
clean:
	for EXT in ${EXTS}; do \
	  find `pwd` -name \*\.$${EXT} -exec rm -v \{\} \; ; done

##show PDF
display: $(TARGET).pdf
	acroread $(TARGET).pdf &

### misc
.SUFFIXES: .tex .aux .toc .lof .lot .log .dvi .dvi2 .ps .ps2 .pdf .bib .bbl


==> parts/wellbeing/priorArt.tex <==
\chapter{Prior Art in Wellbeing Monitoring}\label{ch:wellbeingprior}

\section{Data}



\section{Related Work}



\section{Open Challenges and Opportunities}

...

Hence, this thesis part focuses on the contributions aiming to bring wellbeing monitoring to intelligent vehicles, especially for autonomous vehicles shared by groups of people. Specifically:
\begin{itemize}
    \item In Chapter~\ref{ch:emotion}, ...
    \item In Chapter~\ref{ch:activity}, ...
\end{itemize}
